The 2020 Census Disclosure Avoidance System TopDown Algorithm

The Census TopDown Algorithm (TDA) is a disclosure avoidance system using differential privacy for privacy-loss accounting. The algorithm ingests the final, edited version of the 2020 Census data and the final tabulation geographic definitions. The algorithm then creates noisy versions of key queries on the data, referred to as measurements, using zero-Concentrated Differential Privacy. Another key aspect of the TDA are invariants, statistics that the Census Bureau has determined, as matter of policy, to exclude from the privacy-loss accounting. The TDA post-processes the measurements together with the invariants to produce a Microdata Detail File (MDF) that contains one record for each person and one record for each housing unit enumerated in the 2020 Census. The MDF is passed to the 2020 Census tabulation system to produce the 2020 Census Redistricting Data (P.L. 94-171) Summary File. This paper describes the mathematics and testing of the TDA for this purpose.

==> new_material/TDA_summary.tex <==
%OBSOLETE replaced by TDA Summary Table

\noindent {\bf The TopDown Algorithm summary:}

Measurement Phase
\begin{enumerate}
    \item For $\text{level } i \in \{\text{US}, \text{state}, \text{county}, \text{tract}, \text{block group}, \text{block}\}$
    \begin{enumerate}
        \item Determine the privacy-loss budget for the level $i$
        \item Take differentially private measurements $\widetilde{\mathbf{M}}_{\gamma}$ for all nodes in level $i$
    \end{enumerate}
\end{enumerate}

Estimation Phase
\begin{enumerate}
    \item For the US root node $\gamma_0$ estimate the contingency table vector $\mathbf{x}_{\gamma_0}$ by
    \begin{enumerate}
        \item Estimating a non-negative solution $\tilde{\mathbf{x}}_{\gamma_0}$ from the set of differentially private measurements $\widetilde{\mathbf{M}}_{\gamma_0}$, invariants, and edit constraints at the US level.
        \item Estimating a non-negative integer solution $\hat{\mathbf{x}}_{\gamma_0}$ from $\tilde{\mathbf{x}}_{\gamma_0}$ by controlled rounding. 
    \end{enumerate}
    \item For $\text{level } i \in \{\text{state}, \text{county}, \text{tract}, \text{block group}, \text{block}\}$
    \begin{enumerate}
        \item Let 
        % Note: comment 29
        %$\rho_i$
        $P_i$
        represent the set of distinct parents among all nodes at level $i$. For each parent node %$\gamma \in \rho_i$, 
        $\gamma\in P_i$,
        estimate the joint contingency table vector $\mathbf{x}_{\text{children}(\gamma)}$ by 
        \begin{enumerate}
            \item Estimating a non-negative solution $\tilde{\mathbf{x}}_{\text{children}(\gamma)}$ from the set of differentially private measurements $\widetilde{\mathbf{M}}_{\text{children}(\gamma)}$, invariants, edit constraints, and aggregate constraints enforcing that the children sum to $\hat{\mathbf{x}}_{\gamma}$.
            \item Estimating a non-negative integer solution $\hat{\mathbf{x}}_{\text{children}(\gamma)}$ from $\tilde{\mathbf{x}}_{\text{children}(\gamma)}$ by controlled rounding. 
        \end{enumerate}
    \end{enumerate}
\end{enumerate}

%In each table $T_{\nnode}$ associated with a geography node $\nnode \in \ngeo$, we assume there is \emph{geographic identifier} or \emph{geoid} which uniquely identifies the corresponding geographic location.
%In particular, substrings of each record's geoid column can be used to uniquely identify that geographic node (e.g. the leading $3$ digits of the geoid for each record are used to identify the US state in which that record resides, and also the geographic node corresponding to that state, while the first leading digit is always $0$ and refers to the nation \& node $\nroot$). We refer to the set of all nodes at a fixed distance from $\nroot$ as a \emph{geographic level}, which in the case of the Census may be one of the Nation, States, Counties, Tracts, Block-groups, or Blocks.

% from other paper (would need to track down functions)

% \begin{algorithm}[!ht]
%     \SetKwProg{Fn}{function}{\string:}{}
%     \SetKwFunction{tdb}{TopDownPostprocess}
%     \SetKwFunction{meas}{GetMeasurements}
%     \SetKwFunction{driver}{Driver}
%     \SetKwInOut{Input}{input}
%     \DontPrintSemicolon
%     \Fn{\driver{$\ntable,\set{\nquery_{\nnode}}_{\nnode\in\ngeo}, \epsilon$}}{
%       $\set{\nmeas_{\nnode}}_{\nnode\in\ngeo} \gets \meas(\ntable, \set{\nquery_{\nnode}}_{\nnode\in\ngeo},\epsilon)$\;
%       $\nouttable \gets \tdb(\set{\nquery_{\nnode}}_{\nnode\in\ngeo}, \set{\nmeas_{\nnode}}_{\nnode\in\ngeo})$\;
%       \Return $\nouttable$
%     }
%     \Fn{\meas{$\ntable,\set{\nquery_{\nnode}}_{\nnode\in\ngeo}, \epsilon$}}{
%        $s \gets \sens{\set{\nquery_{\nnode}}_{\nnode\in\ngeo}}$\;
    
%        %\eIf{$\set{\nquery_{\nnode}}_{\nnode\in\ngeo}$ satisfies the Count Condition}{
%            \For{each $\nnode\in\ngeo$}{
%               obtain $\nhist_{\nnode}$ from $\ntable$\;
%               $\nmeas_{\nnode}\gets \nquery_{\nnode} \nhist_{\nnode} + \dgeo(\epsilon/s)$ \tcc{Vector of independent double geometric noise}
%            %}
%        } %ELSE
%        %{
%        %    \For{each $\nnode\in\ngeo$}{
%        %       obtain $\nhist_{\nnode}$ from $\ntable$\;
%        %       $\nmeas_{\nnode}\gets \nquery_{\nnode} \nhist_{\nnode} + \lap(s/\epsilon)$ \tcc{Vector of independent Laplace noise}
%        %    }
    
%        %}
%        \Return $\set{\nmeas_{\nnode}}_{\nnode\in\ngeo}$
%     }
%     \Fn{\tdb{$\set{\nquery_{\nnode}}_{\nnode\in\ngeo}, \set{\nmeas_{\nnode}}_{\nnode\in\ngeo}$}}{
%     node-queue $\gets\emptyset$\;
%     $\mathbf{y}_{\nroot}\gets \arg\min_{\mathbf{y}} ||\nquery_{\nroot}\mathbf{y} - \nmeas_{\nnode}||_2^2$ s.t. $\mathbf{y}\succeq \mathbf{0}$\;
%     $\noutput_{\nroot}\gets \arg\min_{\noutput_{\nroot}} ||\mathbf{y}_{\nroot}-\noutput_{\nroot}||_1$ s.t. $\noutput_{\nroot}\succeq \mathbf{0}$ and $\noutput_{\nroot}$ is integer-valued and $||\nmeas_{\nroot}-\mathbf{y}_{\nroot}||_\infty \leq 1$  and $\mathbf{1}^T \mathbf{y}_{\nroot} = \mathbf{1}^T\noutput_{\nroot}$\;
%     node-queue.append($\nroot$)\;
%     \While{node-queue is not empty}{
%       $\nnode \gets $node-queue.pop()\;
%       $k \gets |\nchild(\nnode)|$\;
%       $\alpha_1,\dots, \alpha_k \gets \nchild(\nnode)$\;
%       $\mathbf{y}_{1},\dots,\mathbf{y}_{k} \gets \arg\min\limits_{\mathbf{y}_{1},\dots,\mathbf{y}_{k}} \sum\limits_{i=1}^k ||\nquery_{\alpha_i}\mathbf{y}_i - \nmeas_{\alpha_i}||_2^2$ s.t. $\mathbf{y}_1,\dots,\mathbf{y}_k\succeq \mathbf{0}$ and $\sum_{i=1}^k \mathbf{y_i}=\noutput_{\nnode}$\;
%     $\noutput_{\alpha_1},\dots, \noutput_{\alpha_k}\gets \arg\min\limits_{\noutput_{\alpha_1},\dots,\noutput_{\alpha_k}} \sum\limits_{i=1}^k ||\mathbf{y}_{i}-\noutput_{\alpha_i}||_1$
%     s.t. $\noutput_{\alpha_1},\dots,\noutput_{\alpha_k}\succeq \mathbf{0}$ and $\noutput_{\alpha_i}$ is integer-valued for every $i$ and $\sum_{i=1}^k \noutput_{\alpha_i}=\noutput_{\nnode}$ and $||\mathbf{y}_i-\noutput_{\alpha_i}||_\infty \leq 1$ for all $i$\;
%     %and  $\mathbf{1}^T \mathbf{y}_{i} = \mathbf{1}^T\noutput_{\alpha_i}$ for all $i$\;
%     \For{each $\alpha_i$}{
%        \If{$\alpha_i$ has children}{
%           node-queue.append($\alpha_1$)
%        }
%       }
%     }
%      Reassemble $\nouttable$ from $\set{\noutput_{\nnode}}_{\nnode\in \ngeo}$\;
%      \Return $\nouttable$
%     }
%     \caption{Basic TopDown Algorithm \label{alg:tdb}}
%     \end{algorithm}

==> new_material/april_experiemnts.tex <==
%l2_optimization_approach = DataIndUserSpecifiedQueriesNPass
%rounder_optimization_approach = MultipassRounder
%DataIndNPass_toleranceType = opt_tol
%#const_tol_val = 25.0
%opt_tol_slack = 0.1

%seq_optimization_approach = L2PlusRounderWithBackup_interleaved

%dp_mechanism =discrete_gaussian_mechanism

%strategy = Strategy1b_St_Cty_BG_optSpine_ppmfCandidate
%query_ordering = Strategy1b_ST_CTY_BG_isoTot_Ordering

%[constraints]
%#the invariants created, (no spaces)
%theInvariants.Block = gqhh_vect, gqhh_tot
%theInvariants.State = tot

%theConstraints.Block = hhgq_total_lb, hhgq_total_ub, nurse_nva_0

class Strategy1b_St_Cty_BG_optSpine_ppmfCandidate:
    @staticmethod
    def make(levels):
        geos_qs_props_dict = defaultdict(lambda: defaultdict(dict))
        geos_qs_props_dict.update({
            CC.GEODICT_GEOLEVELS: levels,
        })
        for level in geos_qs_props_dict[CC.GEODICT_GEOLEVELS]:
            if level == "US": # No 'total' query
                geos_qs_props_dict[CC.DPQUERIES][level] = ("cenrace", "hispanic", "votingage", "hhinstlevels",
                                                            "hhgq", "hispanic * cenrace", "votingage * cenrace",
                                                            "votingage * hispanic", "votingage * hispanic * cenrace", "detailed")
                geos_qs_props_dict[CC.QUERIESPROP][level] = (Fr(1,512), Fr(1,1024), Fr(1,1024), Fr(1,1024),
                                                        Fr(1,1024), Fr(5,1024), Fr(5,1024), Fr(1,1024), Fr(17,1024), Fr(990,1024))
            elif level == "State": # In Redistricting, separately tuned rho on 'total'
                geos_qs_props_dict[CC.DPQUERIES][level] = ("total", "cenrace", "hispanic", "votingage", "hhinstlevels",
                                                            "hhgq", "hispanic * cenrace", "votingage * cenrace",
                                                            "votingage * hispanic", "votingage * hispanic * cenrace", "detailed")
                geos_qs_props_dict[CC.QUERIESPROP][level] = (Fr(678,1024),Fr(1,1024),Fr(1,1024),Fr(1,1024),
                                                            Fr(1,1024),Fr(1,1024),Fr(2,1024),Fr(2,1024),
                                                            Fr(1,1024),Fr(6,1024),Fr(330,1024))
            elif level == "County": # In Redistricting, separately tuned rho on 'total'
                geos_qs_props_dict[CC.DPQUERIES][level] = ("total", "cenrace", "hispanic", "votingage", "hhinstlevels",
                                                            "hhgq", "hispanic * cenrace", "votingage * cenrace",
                                                            "votingage * hispanic", "votingage * hispanic * cenrace", "detailed")
                geos_qs_props_dict[CC.QUERIESPROP][level] = (Fr(342,1024), Fr(1,1024), Fr(1,1024), Fr(1,1024), Fr(1,1024),
                                                        Fr(1,1024), Fr(3,1024), Fr(3,1024), Fr(1,1024), Fr(11,1024), Fr(659,1024))
            elif level == "Block_Group":
                geos_qs_props_dict[CC.DPQUERIES][level] = ("total", "cenrace", "hispanic", "votingage", "hhinstlevels",
                                                            "hhgq", "hispanic * cenrace", "votingage * cenrace",
                                                            "votingage * hispanic", "votingage * hispanic * cenrace", "detailed")
                geos_qs_props_dict[CC.QUERIESPROP][level] = (Fr(572,1024), Fr(1,1024), Fr(1,1024), Fr(1,1024), Fr(1,1024),
                                                        Fr(1,1024), Fr(3,1024), Fr(3,1024), Fr(1,1024), Fr(8,1024), Fr(432,1024))
            else: # Only per-geolevel rho actively tuned in other geolevels; query allocations left at default
                geos_qs_props_dict[CC.DPQUERIES][level] = ("total", "cenrace", "hispanic", "votingage", "hhinstlevels",
                                                            "hhgq", "hispanic * cenrace", "votingage * cenrace",
                                                            "votingage * hispanic", "votingage * hispanic * cenrace", "detailed")
                geos_qs_props_dict[CC.QUERIESPROP][level] = (Fr(1,1024), Fr(1,512), Fr(1,1024), Fr(1,1024), Fr(1,1024),
                                                        Fr(1,1024), Fr(5,1024), Fr(5,1024), Fr(1,1024), Fr(17,1024), Fr(989,1024))
        return geos_qs_props_dict
        
        
        
        
class Strategy1b_ST_CTY_BG_isoTot_Ordering:
    @staticmethod
    def make(levels):
        # levels = USGeolevelsNoTractGroup.getLevels()
        us_ordering = {
            CC.L2_QUERY_ORDERING: {
                0: {
                    0: ('cenrace', 'hispanic', 'votingage', 'hhinstlevels', 'hhgq', 'votingage * hispanic',
                        'hispanic * cenrace', 'votingage * cenrace',
                        'votingage * hispanic * cenrace', 'detailed'),
                },
            },
            CC.L2_CONSTRAIN_TO_QUERY_ORDERING: {
                0: {
                    0: ('cenrace', 'hispanic', 'votingage', 'hhinstlevels', 'hhgq', 'votingage * hispanic',
                        'hispanic * cenrace', 'votingage * cenrace',
                        'votingage * hispanic * cenrace', 'detailed'),
                },
            },
            CC.ROUNDER_QUERY_ORDERING: {
                0: {
                    0: ('total', 'hhgq', 'hhgq * hispanic', 'hhgq * hispanic * cenrace', 'hhgq * votingage * hispanic * cenrace',
                        'detailed'),
                },
            },
        }
        st_cty_bg_ordering = {
            CC.L2_QUERY_ORDERING: {
                0: {
                    0: ('total',),
                    1: ('cenrace', 'hispanic', 'votingage', 'hhinstlevels', 'hhgq', 'votingage * hispanic',
                        'hhgq', 'hispanic * cenrace', 'votingage * cenrace', 'votingage * hispanic',
                        'votingage * hispanic * cenrace',
                        'detailed'),
                },
            },
            CC.L2_CONSTRAIN_TO_QUERY_ORDERING: {
                0: {
                    0: ('total',),
                    1: ('cenrace', 'hispanic', 'votingage', 'hhinstlevels', 'hhgq', 'votingage * hispanic',
                        'hhgq', 'hispanic * cenrace', 'votingage * cenrace', 'votingage * hispanic',
                        'votingage * hispanic * cenrace',
                        'detailed'),
                },
            },

            CC.ROUNDER_QUERY_ORDERING: {
                0: {
                    0: ('total',),
                    1: ('hhgq', 'hhgq * hispanic', 'hhgq * hispanic * cenrace', 'hhgq * votingage * hispanic * cenrace',
                        'detailed'),
                },
            },
        }
        default_ordering = {
            CC.L2_QUERY_ORDERING: {
                0: {
                    0: ('total', 'cenrace', 'hispanic', 'votingage', 'hhinstlevels', 'hhgq', 'votingage * hispanic',
                        'hhgq', 'hispanic * cenrace', 'votingage * cenrace', 'votingage * hispanic',
                        'votingage * hispanic * cenrace', 'detailed'),
                },
            },
            CC.L2_CONSTRAIN_TO_QUERY_ORDERING: {
                0: {
                    0: ('total', 'cenrace', 'hispanic', 'votingage', 'hhinstlevels', 'hhgq', 'votingage * hispanic',
                        'hhgq', 'hispanic * cenrace', 'votingage * cenrace', 'votingage * hispanic',
                        'votingage * hispanic * cenrace', 'detailed'),
                },
            },
            CC.ROUNDER_QUERY_ORDERING: {
                0: {
                    0: ('total', 'hhgq', 'hhgq * hispanic', 'hhgq * hispanic * cenrace', 'hhgq * votingage * hispanic * cenrace',
                        'detailed'),
                },
            },
        }

        query_ordering = {}
        for geolevel in levels:
            if geolevel == "US":
                query_ordering[geolevel] = us_ordering
            elif geolevel in ("State", "County", "Block_Group"):
                query_ordering[geolevel] = st_cty_bg_ordering
            else:
                query_ordering[geolevel] = default_ordering
        return query_ordering
